Understanding Practical Optimization in Machine Learning

Modern machine learning relies on practical optimization methods that often differ from the algorithms studied in classical analyses: they train submodels, clip or normalize gradients, use layer-wise non-Euclidean directions, or approximate costly inner computations. This thesis analyzes the objective, assumptions, update, and computation defined by these procedures, rather than those of simplified proxies. For submodel training, we show that Independent Subnetwork Training can converge to a shifted fixed point because sketching before differentiation biases the update for the original objective. Model-Agnostic Sparsified Training instead incorporates the sketch distribution into its objective, which makes sketched gradients unbiased and admits convergence guarantees. For private optimization, we show that adaptive quantile clipping retains bias at any fixed quantile, while suitable quantile schedules recover near-optimal nonconvex rates under heavy-tailed noise. We then combine smoothed normalization with error compensation and obtain distributed private convergence guarantees under standard assumptions, without assuming bounded gradients. For optimizers based on linear minimization oracles, we develop and validate a layer-wise generalized smoothness model and build on it the Gluon framework for Muon- and Scion-style methods. We also show that the approximate orthogonalization in Muon matters: less precise orthogonalization calls for smaller stepsizes, so its precision should be tuned together with the learning rate. Overall, practical methods are better understood when theory retains the features that determine their optimization behavior.

==> KAUST_Thesis/imported/02_ist/import_setup.tex <==
%
%
\makeatletter
\let\egor\@undefined
\let\peter\@undefined
\let\as\@undefined
\let\asnote\@undefined
\let\libname\@undefined
\let\algname\@undefined
\let\DCGD\@undefined
\let\DIANA\@undefined
\let\GDCI\@undefined
\let\AG\@undefined
\let\finf\@undefined
\let\prox\@undefined
\let\range\@undefined
\let\Comp\@undefined
\let\Comm\@undefined
\let\Span\@undefined
\let\Sp\@undefined
\let\Diag\@undefined
\let\diag\@undefined
\let\tr\@undefined
\let\cDb\@undefined
\let\Exp\@undefined
\let\ExpSub\@undefined
\let\ExpCond\@undefined
\let\bg\@undefined
\let\Rd\@undefined
\let\R\@undefined
\let\eps\@undefined
\let\Dotprod\@undefined
\let\norm\@undefined
\let\sqn\@undefined
\let\Norm\@undefined
\let\sqN\@undefined
\let\vect\@undefined
\let\ecn\@undefined
\let\cR\@undefined
\let\cG\@undefined
\let\cV\@undefined
\let\cE\@undefined
\let\cL\@undefined
\let\cC\@undefined
\let\cQ\@undefined
\let\cZ\@undefined
\let\cY\@undefined
\let\cX\@undefined
\let\sX\@undefined
\let\cO\@undefined
\let\cT\@undefined
\let\Lag\@undefined
\let\mA\@undefined
\let\mB\@undefined
\let\mC\@undefined
\let\mD\@undefined
\let\mE\@undefined
\let\mV\@undefined
\let\mW\@undefined
\let\mL\@undefined
\let\mZ\@undefined
\let\mI\@undefined
\let\mP\@undefined
\let\mM\@undefined
\let\mWp\@undefined
\let\bN\@undefined
\let\bU\@undefined
\let\bC\@undefined
\let\bB\@undefined
\let\bR\@undefined
\let\sqnw\@undefined
\let\eqdef\@undefined
\let\br\@undefined
\let\sbr\@undefined
\let\cbr\@undefined
\let\bfL\@undefined
\let\bfC\@undefined
\let\mcL\@undefined
\let\mcB\@undefined
\let\cb\@undefined
\let\moL\@undefined
\let\moB\@undefined
\let\moD\@undefined
\let\moW\@undefined
\let\ob\@undefined
\let\oCb\@undefined
\let\bb\@undefined
\let\oDb\@undefined
\let\cbb\@undefined
\let\E\@undefined
\let\EE\@undefined
\let\Var\@undefined
\let\argmin\@undefined
\makeatother
\input{KAUST_Thesis/imported/02_ist/source_macros}
%
%
\newcommand{\istord}[1]{\mathord{#1}}
\renewcommand{\bfL}{\istord{\mathbf{L}}}
\renewcommand{\bfC}{\istord{\mathbf{C}}}
\renewcommand{\mcL}{\istord{\tilde{\mathbf{L}}}}
\renewcommand{\mcB}{\istord{\tilde{\mathbf{B}}}}
\renewcommand{\cb}{\istord{\tilde{\mathrm{b}}}}
\renewcommand{\moL}{\istord{\overline{\mathbf{L}}}}
\renewcommand{\moB}{\istord{\overline{\mathbf{B}}}}
\renewcommand{\moD}{\istord{\overline{\mathbf{D}}}}
\renewcommand{\moW}{\istord{\overline{\mathbf{W}}}}
\renewcommand{\ob}{\istord{\overline{b}}}
\renewcommand{\oCb}{\istord{\overline{\mathbf{C}b}}}
\renewcommand{\bb}{\istord{\mathrm{b}}}
\renewcommand{\oDb}{\istord{\overline{\mD^{-\frac{1}{2}}\bb}}}
\renewcommand{\cbb}{\istord{\overline{\bb^{\frac{1}{2}}}}}
\makeatletter
\let\theHalgorithm\@undefined
\makeatother
\newcommand{\theHalgorithm}{\arabic{algorithm}}
\providecommand{\say}[1]{``#1''}
\makeatletter
\providecommand{\import@cite@plain}[1]{\cite{#1}}
\providecommand{\import@cite@opt}[1][]{\@ifnextchar[{\import@cite@opt@two}{\import@cite@opt@one}}
\providecommand{\import@cite@opt@one}[1]{\cite{#1}}
\providecommand{\import@cite@opt@two}[2][]{\cite{#2}}
\@ifundefined{citep}{\DeclareRobustCommand{\citep}{\@ifnextchar[{\import@cite@opt}{\import@cite@plain}}}{}
\@ifundefined{citet}{\DeclareRobustCommand{\citet}{\citep}}{}
\@ifundefined{citealp}{\DeclareRobustCommand{\citealp}{\citep}}{}
\@ifundefined{citealt}{\DeclareRobustCommand{\citealt}{\citep}}{}
\@ifundefined{citeauthor}{\DeclareRobustCommand{\citeauthor}{\citep}}{}
\@ifundefined{citeyear}{\DeclareRobustCommand{\citeyear}{\citep}}{}
\@ifundefined{citeyearpar}{\DeclareRobustCommand{\citeyearpar}{\citep}}{}
\makeatother
\providecommand{\Cref}[1]{\ref{#1}}
\providecommand{\cref}[1]{\ref{#1}}
\providecommand{\squeeze}{\textstyle}
\def\<#1,#2>{\langle #1,#2\rangle}


==> KAUST_Thesis/imported/02_ist/source_macros.tex <==
%
%
%
%
%

%
%
%
%
%
%


%
%
%
%
%
%
%
%
%

%
%

%
%
%
%

%

%

%
%

\newcommand{\egor}[1]{\todo[inline]{\footnotesize \textbf{Egor:} #1}}
\newcommand{\peter}[1]{\todo[inline]{\footnotesize Peter: #1}}

\newcommand{\as}[1]{{\color{green} #1}}
\newcommand{\asnote}[1]{\todo[color=green!]{#1}}

%

%
%
\newcommand{\algname}[1]{{\sf#1}\xspace}

\newcommand{\DCGD}{\algname{DCGD}}
\newcommand{\DIANA}{\algname{DIANA}}
\newcommand{\GDCI}{\algname{GDCI}}

%
%
%
%
%
%

\newcommand{\AG}{\mathrm{AG}}

\newcommand{\finf}{f^{\mathrm{inf}}}

\newcommand{\prox}{\mathrm{prox}}
\newcommand{\range}{\mathrm{range}}
\newcommand{\Comp}{\mathrm{Comp}}
\newcommand{\Comm}{\mathrm{Comm}}
\newcommand{\Span}{\mathrm{Span}}
\newcommand{\Sp}{\mathrm{Sp}}

\newcommand{\Diag}{\mathrm{Diag}}
\newcommand{\diag}{\mathrm{diag}}

\newcommand{\tr}{\mathrm{tr}}

\newcommand{\bfL}{\mathop{\mathbf{L}}}
\newcommand{\bfC}{\mathop{\mathbf{C}}}
\newcommand{\mcL}{\mathop{\tilde{\mathbf{L}}}}
\newcommand{\mcB}{\mathop{\tilde{\mathbf{B}}}}
\newcommand{\cb}{\mathop{\tilde{\mathrm{b}}}}

\newcommand{\moL}{\mathop{\overline{\mathbf{L}}}}
\newcommand{\moB}{\mathop{\overline{\mathbf{B}}}}
\newcommand{\moD}{\mathop{\overline{\mathbf{D}}}}
\newcommand{\moW}{\mathop{\overline{\mathbf{W}}}}
\newcommand{\ob}{\mathop{\overline{b}}}
\newcommand{\oCb}{\mathop{\overline{\mathbf{C}b}}}

\newcommand{\bb}{\mathop{\mathrm{b}}}
\newcommand{\oDb}{\mathop{\overline{\mD^{-\frac{1}{2}}\bb}}}
\newcommand{\cDb}{\widetilde{\mD\bb}}
\newcommand{\cbb}{\mathop{\overline{\bb^{\frac{1}{2}}}}}


\newcommand{\E}{\mathop{\mathbb{E}}}
\newcommand{\EE}{\mathop{\mathbb{E}}}
\newcommand{\Exp}[1]{{\color{black}  \mathbb{E}}\left[#1\right]}
\newcommand{\ExpSub}[2]{{\mathbb{E}}_{#1}\left[#2\right]}
\newcommand{\ExpCond}[2]{{\mathbb{E}}\left[\left.#1\right\vert#2\right]}
\newcommand{\Var}{\mathop{{\bf Var}}}

\newcommand{\bg}{\mathrm{D}}

\newcommand{\Rd}{\mathbb{R}^d}
\newcommand{\R}{\ensuremath{\mathbb{R}}}

\newcommand{\eps}{\varepsilon}

\def\<#1,#2>{\langle #1,#2\rangle}

\newcommand{\Dotprod}[1]{\left\langle#1\right\rangle}


\newcommand{\norm}[1]{\|#1\|}
\newcommand{\sqn}[1]{\norm{#1}^2}
\newcommand{\Norm}[1]{\left\|#1\right\|}
\newcommand{\sqN}[1]{\Norm{#1}^2}
\newcommand{\vect}[1]{\begin{bmatrix*}[l]#1\end{bmatrix*}}
\newcommand{\ecn}[1]{\Exp{\sqn{#1}}}
\newcommand\br[1]{\left ( #1 \right )}
\newcommand\sbr[1]{\left[#1\right]}
\newcommand\cbr[1]{\left\{#1\right\}}


\newcommand{\cR}{\mathcal{R}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\sX}{{\mathsf E}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\Lag}{\mathcal{L}}

\newcommand{\mA}{\mathbf{A}}
\newcommand{\mB}{\mathbf{B}}
\newcommand{\mC}{\mathbf{C}}
\newcommand{\mD}{\mathbf{D}}
\newcommand{\mE}{\mathbf{E}}
\newcommand{\mV}{\mathbf{V}}
\newcommand{\mW}{\mathbf{W}}
\newcommand{\mL}{\mathbf{L}}
\newcommand{\mZ}{\mathbf{Z}}
\newcommand{\mI}{\mathbf{I}}
\newcommand{\mP}{\mathbf{P}}
%


\newcommand{\mM}{\mathbf{M}}
\newcommand{\mWp}{\mathbf{W}^{\dagger}}



\newcommand{\bN}{\mathbb{N}}
\newcommand{\bU}{\mathbb{U}}
\newcommand{\bC}{\mathbb{C}}
\newcommand{\bB}{\mathbb{B}}
\newcommand{\bR}{\mathbb{R}}

\newcommand{\sqnw}[1]{\sqn{#1}_{\mWp}}
\newcommand{\eqdef}{\coloneqq}
\newcommand{\argmin}{\operatorname*{arg\,min}}


==> KAUST_Thesis/imported/03_mast/import_setup.tex <==
%
%
\makeatletter
\let\Arg\@undefined
\let\Corr\@undefined
\let\Cov\@undefined
\let\Ctk\@undefined
\let\D\@undefined
\let\Diag\@undefined
\let\E\@undefined
\let\Exp\@undefined
\let\ExpSub\@undefined
\let\Image\@undefined
\let\Ker\@undefined
\let\La\@undefined
\let\MVEE\@undefined
\let\Prob\@undefined
\let\R\@undefined
\let\SGD\@undefined
\let\Var\@undefined
\let\ahnorm\@undefined
\let\al\@undefined
\let\alg\@undefined
\let\algname\@undefined
\let\anorm\@undefined
\let\approxalg\@undefined
\let\argmax\@undefined
\let\argmin\@undefined
\let\bA\@undefined
\let\bB\@undefined
\let\bC\@undefined
\let\bD\@undefined
\let\bE\@undefined
\let\bG\@undefined
\let\bI\@undefined
\let\bL\@undefined
\let\bLa\@undefined
\let\bM\@undefined
\let\bN\@undefined
\let\bP\@undefined
\let\bU\@undefined
\let\barB\@undefined
\let\barC\@undefined
\let\barL\@undefined
\let\bb\@undefined
\let\bbone\@undefined
\let\bdry\@undefined
\let\blue\@undefined
\let\bnorm\@undefined
\let\bx\@undefined
\let\by\@undefined
\let\cA\@undefined
\let\cC\@undefined
\let\cCd\@undefined
\let\cCw\@undefined
\let\cD\@undefined
\let\cE\@undefined
\let\cO\@undefined
\let\cQ\@undefined
\let\cS\@undefined
\let\cX\@undefined
\let\card\@undefined
\let\cl\@undefined
\let\cmark\@undefined
\let\cone\@undefined
\let\conv\@undefined
\let\del\@undefined
\let\dfr\@undefined
\let\diag\@undefined
\let\diam\@undefined
\let\dom\@undefined
\let\done\@undefined
\let\egor\@undefined
\let\eik\@undefined
\let\eikpo\@undefined
\let\eit\@undefined
\let\eitpo\@undefined
\let\epi\@undefined
\let\eps\@undefined
\let\eqdef\@undefined
\let\eqtext\@undefined
\let\fiinf\@undefined
\let\finf\@undefined
\let\fr\@undefined
\let\g\@undefined
\let\getext\@undefined
\let\gh\@undefined
\let\ghx\@undefined
\let\gih\@undefined
\let\gihx\@undefined
\let\gik\@undefined
\let\gikpo\@undefined
\let\gixk\@undefined
\let\gnorm\@undefined
\let\green\@undefined
\let\hA\@undefined
\let\hAi\@undefined
\let\hG\@undefined
\let\hS\@undefined
\let\head\@undefined
\let\hg\@undefined
\let\hgi\@undefined
\let\hgik\@undefined
\let\hgikpo\@undefined
\let\hgix\@undefined
\let\hgiy\@undefined
\let\hgu\@undefined
\let\hotidea\@undefined
\let\hs\@undefined
\let\ii\@undefined
\let\interior\@undefined
\let\la\@undefined
\let\lam\@undefined
\let\lami\@undefined
\let\letext\@undefined
\let\lin\@undefined
\let\linspace\@undefined
\let\linspan\@undefined
\let\lmbdM\@undefined
\let\lsvrg\@undefined
\let\lt\@undefined
\let\mB\@undefined
\let\mC\@undefined
\let\mD\@undefined
\let\mI\@undefined
\let\mL\@undefined
\let\mM\@undefined
\let\mN\@undefined
\let\maxi\@undefined
\let\maxin\@undefined
\let\mbf\@undefined
\let\mds\@undefined
\let\mini\@undefined
\let\minin\@undefined
\let\nf\@undefined
\let\nfr\@undefined
\let\norm\@undefined
\let\notneeded\@undefined
\let\nullspace\@undefined
\let\onenorm\@undefined
\let\opn\@undefined
\let\orange\@undefined
\let\p\@undefined
\let\pA\@undefined
\let\pB\@undefined
\let\pC\@undefined
\let\peter\@undefined
\let\ppA\@undefined
\let\ppB\@undefined
\let\ppC\@undefined
\let\preceqtext\@undefined
\let\qedb\@undefined
\let\ra\@undefined
\let\range\@undefined
\let\rank\@undefined
\let\red\@undefined
\let\ri\@undefined
\let\rint\@undefined
\let\rnd\@undefined
\let\rt\@undefined
\let\sarit\@undefined
\let\shift\@undefined
\let\sign\@undefined
\let\signum\@undefined
\let\sqn\@undefined
\let\sqnorm\@undefined
\let\squeeze\@undefined
\let\st\@undefined
\let\stepsize\@undefined
\let\succtext\@undefined
\let\sumid\@undefined
\let\sumin\@undefined
\let\suminn\@undefined
\let\sumjm\@undefined
\let\sumjmi\@undefined
\let\sumjmm\@undefined
\let\sumjmmi\@undefined
\let\sumjn\@undefined
\let\sumjnn\@undefined
\let\sumlmi\@undefined
\let\tf\@undefined
\let\theHalgorithm\@undefined
\let\threenorm\@undefined
\let\todo\@undefined
\let\topic\@undefined
\let\tr\@undefined
\let\twonorm\@undefined
\let\ve\@undefined
\let\vik\@undefined
\let\vikpo\@undefined
\let\vit\@undefined
\let\vitpo\@undefined
\let\vol\@undefined
\let\vp\@undefined
\let\wA\@undefined
\let\wB\@undefined
\let\wC\@undefined
\let\wG\@undefined
\let\wL\@undefined
\let\wLi\@undefined
\let\wS\@undefined
\let\wcC\@undefined
\let\wg\@undefined
\let\wgik\@undefined
\let\wgikpo\@undefined
\let\wgix\@undefined
\let\wgiy\@undefined
\let\wgu\@undefined
\let\wik\@undefined
\let\wikpo\@undefined
\let\wjk\@undefined
\let\wjkpo\@undefined
\let\wk\@undefined
\let\wpA\@undefined
\let\wpB\@undefined
\let\wpC\@undefined
\let\ws\@undefined
\let\wt\@undefined
\let\wwL\@undefined
\let\xmark\@undefined
\let\yura\@undefined
\let\z\@undefined
\let\zerosarah\@undefined
\let\br\@undefined
\let\sbr\@undefined
\let\cbr\@undefined
\makeatother
\input{KAUST_Thesis/imported/03_mast/source_macros}
\makeatletter
\let\tf\@undefined
\let\shift\@undefined
\let\mS\@undefined
\let\squeeze\@undefined
\makeatother
\newcommand{\tf}{f_{\mathcal{D}}}
\newcommand{\shift}{{\color{purple}v}}
\newcommand{\mS}{{\bf S}}
\newcommand{\squeeze}{\textstyle}
\makeatletter
\providecommand{\import@cite@plain}[1]{\cite{#1}}
\providecommand{\import@cite@opt}[1][]{\@ifnextchar[{\import@cite@opt@two}{\import@cite@opt@one}}
\providecommand{\import@cite@opt@one}[1]{\cite{#1}}
\providecommand{\import@cite@opt@two}[2][]{\cite{#2}}
\@ifundefined{citep}{\DeclareRobustCommand{\citep}{\@ifnextchar[{\import@cite@opt}{\import@cite@plain}}}{}
\@ifundefined{citet}{\DeclareRobustCommand{\citet}{\citep}}{}
\@ifundefined{citealp}{\DeclareRobustCommand{\citealp}{\citep}}{}
\@ifundefined{citealt}{\DeclareRobustCommand{\citealt}{\citep}}{}
\@ifundefined{citeauthor}{\DeclareRobustCommand{\citeauthor}{\citep}}{}
\@ifundefined{citeyear}{\DeclareRobustCommand{\citeyear}{\citep}}{}
\@ifundefined{citeyearpar}{\DeclareRobustCommand{\citeyearpar}{\citep}}{}
\makeatother
\providecommand{\Cref}[1]{\ref{#1}}
\providecommand{\cref}[1]{\ref{#1}}
\providecommand{\say}[1]{``#1''}
\providecommand{\todo}[2][]{}
\providecommand{\sfrac}[2]{\nicefrac{#1}{#2}}
\def\<#1,#2>{\langle #1,#2\rangle}


==> KAUST_Thesis/imported/03_mast/source_macros.tex <==
%


%
%

%
%
%

%
%

%

%
%
%
%
%
%
\restylefloat{table}
%

%

%
%
%
%
%
%
%
%

%
%

%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%
%

%


%
%
%

\newcommand\br[1]{\left ( #1 \right )}
\newcommand\sbr[1]{\left[#1\right]}
\newcommand\cbr[1]{\left\{#1\right\}}

\newcommand{\sqn}[1]{\norm{#1}^2}
\newcommand{\rnd}[1]{{\texttt{Rand-}}#1}

\newcommand{\lmbdM}{\lambda_{\mathrm{m}}}


%
%

%
%

\newcommand{\ve}[2]{\left\langle #1 ,  #2 \right\rangle}

%
\newcommand{\cX}{{\cal X}}


%
%

\definecolor{burgundy}{rgb}{0.5, 0.0, 0.13}
\definecolor{darkscarlet}{rgb}{0.34, 0.01, 0.1}
\newcommand{\shift}{{\color{purple}s}} %
\newcommand{\tf}{\tilde{f}}

\newcommand{\SGD}{$\mathsf{SGD}$}
\newcommand{\lsvrg}{$\mathsf{L}$-$\mathsf{SVRG}$~}

%
%

%
%
%

\newcommand{\argmax}{\operatorname*{arg\,max}}
\newcommand{\argmin}{\operatorname*{arg\,min}}
\newcommand{\sign}{\operatorname*{sign}}
%

\newcommand{\z}{\zeta}
\newcommand{\lt}{\left}
\newcommand{\rt}{\right}
\newcommand{\al}{\alpha}
\newcommand{\p}{\partial}
\newcommand{\D}{\Delta}
\newcommand{\nfr}{\nicefrac}
\newcommand{\fr}{\frac}
\newcommand{\dfr}{\dfrac}
\newcommand{\mbf}{\mathbf}
\newcommand{\mds}{\mathds}
\newcommand{\bb}{\mathbb}
\newcommand{\wt}{\widetilde}
\newcommand{\wS}{\wt{S}}
\newcommand{\wA}{\wt{A}}
\newcommand{\wL}{\wt{L}}
\newcommand{\wLi}{\wt{L}_i}
\newcommand{\wwL}{\wt{\wt{L}}}
\newcommand{\wB}{\wt{B}}
\newcommand{\wC}{\wt{C}}
\newcommand{\ws}{\wt{s}}
\newcommand{\wg}{\wt{g}}
\newcommand{\wgix}{\wg_i(x)}
\newcommand{\wgiy}{\wg_i(y)}
\newcommand{\wgik}{\wg_i(x^k)}
\newcommand{\wgikpo}{\wg_i(x^{k+1})}
\newcommand{\wgu}{\wt{g}^u}
\newcommand{\wG}{\wt{G}}
\newcommand{\hG}{\hat{G}}
\newcommand{\hAi}{\hat{A}_i}
\newcommand{\hA}{\hat{A}}
\newcommand{\pA}{A^{\prime}}
\newcommand{\pB}{B^{\prime}}
\newcommand{\pC}{C^{\prime}}
\newcommand{\wpA}{\wA^{\prime}}
\newcommand{\wpB}{\wB^{\prime}}
\newcommand{\wpC}{\wC^{\prime}}
\newcommand{\ppA}{A^{\prime \prime}}
\newcommand{\ppB}{B^{\prime \prime}}
\newcommand{\ppC}{C^{\prime \prime}}


\newcommand{\hg}{\hat{g}}
\newcommand{\hgi}{\hat{g}_i}
\newcommand{\hgix}{\hat{g}_i(x)}
\newcommand{\hgiy}{\hat{g}_i(y)}
\newcommand{\hgik}{\hat{g}_i(x^k)}
\newcommand{\hgikpo}{\hat{g}_i(x^{k+1})}
\newcommand{\hgu}{\hat{g}^u}
\newcommand{\hs}{\hat{s}}


\newcommand{\eik}{e_i^t}
\newcommand{\gik}{g_i^t}
\newcommand{\gikpo}{g_i^{t+1}}
\newcommand{\eikpo}{e_i^{t+1}}
\newcommand{\vik}{v_i^t}
\newcommand{\vikpo}{v_i^{t+1}}

\newcommand{\eit}{e_i^t}
\newcommand{\eitpo}{e_i^{t+1}}
%
%

\newcommand{\wcC}{\wt{\cC}}
\newcommand{\La}{\Lambda}
\newcommand{\lam}{\lambda}
\newcommand{\lami}{\lam_i}
\newcommand{\opn}{\operatorname}
\newcommand{\vp}{\varphi}
\newcommand{\bM}{\mbf M}
\newcommand{\bG}{\mbf G}
\newcommand{\bI}{\mbf I}
\newcommand{\bD}{\mbf D}
\newcommand{\bA}{\mbf A}
\newcommand{\bC}{\mbf C}
\newcommand{\bP}{\mbf P}
\newcommand{\bB}{\bb B}
\newcommand{\bU}{\bb U}
\newcommand{\bLa}{\mbf {\La}}
\newcommand{\R}{\bb R}
\newcommand{\bE}{\mbf E}
\newcommand{\hS}{\hat{S}}
\newcommand{\eps}{{\varepsilon}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\stepsize}{\eta}
\newcommand{\cE}{{\cal E}}
\newcommand{\norm}[1]{\left\| #1 \right\|}
\newcommand{\lin}[1]{\left\langle #1\right\rangle} %
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cCw}{\cC_{\omega}}
\newcommand{\cCd}{\cC_{\delta}}
\newcommand{\Ctk}[1]{\cC_{Tk}\rb{#1}}
\newcommand{\gixk}{g_{i}(x_k)}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\mM}{\mathbf{M}}
\newcommand{\mN}{\mathbf{N}}
\newcommand{\bN}{\mathbf{N}}
\newcommand{\mI}{\mathbf{I}}
\newcommand{\mL}{\mathbf{L}}
\newcommand{\mD}{\mathbf{D}}
\newcommand{\bx}{\bar{x}}
\newcommand{\by}{\bar{y}}
\newcommand{\barB}{\overline{B}}
\newcommand{\barL}{\overline{L}}
\newcommand{\barC}{\overline{C}}
\newcommand{\eqtext}[1]{\ensuremath{\stackrel{\text{#1}}{=}}}
\newcommand{\letext}[1]{\ensuremath{\stackrel{\text{#1}}{\le}}}
\newcommand{\getext}[1]{\ensuremath{\stackrel{\text{#1}}{\ge}}}
\newcommand{\succtext}[1]{\ensuremath{\stackrel{\text{#1}}{\succ}}}
\newcommand{\preceqtext}[1]{\ensuremath{\stackrel{\text{#1}}{\preceq}}}
\newcommand{\onenorm}[1]{\left\| #1 \right\|_1}      %
\newcommand{\twonorm}[1]{\left\| #1 \right\|_2}      %
\newcommand{\threenorm}[1]{\left\| #1 \right\|_3}      %
\newcommand{\gnorm}[1]{\left\| #1 \right\|^{1 + \gamma }}      %
\newcommand{\sqnorm}[1]{\left\| #1 \right\|^{2}}
\newcommand{\anorm}[1]{\left\| #1 \right\|^{\al}}      %
\newcommand{\bnorm}[1]{\left\| #1 \right\|^{\beta}}      %
\newcommand{\ahnorm}[1]{\left\| #1 \right\|^{\al/2}}      %
\newcommand{\bbone}[1]{\mathbb{1}}      %
\newcommand{\g}{\gamma}

\newcommand{\nf}[1]{\nabla f\rb{#1}}      %

\newcommand{\hotidea}{{\color{red}\bf HOT IDEA: }}
\newcommand{\done}{{\color{blue}\bf DONE: }}
\newcommand{\cO}{{\cal O}}

\newcommand{\del}[1]{}

\newcommand{\finf}{f^\mathrm{inf}}
\newcommand{\fiinf}{f_i^\mathrm{inf}}

\let\la=\langle
\let\ra=\rangle

\def\<{\left\langle}
\def\>{\right\rangle}
%
%
\def\({\left(}
\def\){\right)}

%


\newcommand{\eqdef}{\stackrel{\text{def}}{=}}

\newcommand{\ii}{{}^{(i)}}


\newcommand{\Prob}{\mathbf{Prob}}
\newcommand{\E}{\mathbb{E}}



%
\newcommand{\card}{\operatorname{card}}
\newcommand{\diam}{\operatorname{diam}}
\newcommand{\MVEE}{\operatorname{MVEE}}
\newcommand{\vol}{\operatorname{vol}}

%
%
%
\newcommand{\Exp}[1]{{\mathbb{E}}\left[#1\right]}
\newcommand{\ExpSub}[2]{{\mathbb{E}}_{#1}\left[#2\right]}

\newcommand{\Cov}{\operatorname{Cov}}
\newcommand{\Var}{\operatorname{Var}}
\newcommand{\Corr}{\operatorname{Corr}}

%
\newcommand{\signum}{\operatorname{sign}}
\newcommand{\dom}{\operatorname{dom}}
\newcommand{\epi}{\operatorname{epi}}
\newcommand{\Ker}{\operatorname{null}}
\newcommand{\nullspace}{\operatorname{null}}
\newcommand{\range}{\operatorname{range}}
\newcommand{\Image}{\operatorname{Im}}

%
\newcommand{\interior}{\operatorname{int}}
\newcommand{\ri}{\operatorname{rint}}
\newcommand{\rint}{\operatorname{rint}}
\newcommand{\bdry}{\operatorname{bdry}}
\newcommand{\cl}{\operatorname{cl}}

%
\newcommand{\linspan}{\operatorname{span}}
\newcommand{\linspace}{\operatorname{linspace}}
\newcommand{\cone}{\operatorname{cone}}

%
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\conv}{\operatorname{conv}}
\newcommand{\Diag}{\operatorname{Diag}}
\newcommand{\diag}{\operatorname{diag}}

\newcommand{\Arg}{\operatorname{Arg}}



\newcommand {\maxin}{\max_{i=1,\dots, n}}
\newcommand {\maxi}{\max_{i}}
\newcommand {\minin}{\min_{i=1,\dots, n}}
\newcommand {\mini}{\min_{i}}
\newcommand {\sumin}{\sum_{i=1}^{n}}
\newcommand {\sumlmi}{\fr{1}{m_i}\sum_{l=1}^{m_i}}
\newcommand {\suminn}{\fr{1}{n}\sum_{i=1}^{n}}
\newcommand {\sumjm}{\sum_{j=1}^{m}}
\newcommand {\sumjmi}{\sum_{j=1}^{m_i}}
\newcommand {\sumjmm}{\fr{1}{m}\sum_{j=1}^{m}}
\newcommand {\sumjnn}{\fr{1}{n}\sum_{j=1}^{n}}
\newcommand {\sumjmmi}{\fr{1}{m_i}\sum_{j=1}^{m_i}}
\newcommand {\sumjn}{\sum_{j=1}^{n}}
\newcommand {\wik}{w_{i}^{k}}
\newcommand {\wjk}{w_{j}^{k}}
\newcommand {\wk}{w^{k}}
\newcommand {\wikpo}{w_{i}^{k+1}}
\newcommand {\wjkpo}{w_{j}^{k+1}}
%
\newcommand {\sumid}{\sum_{i=1}^{d}}
\newcommand {\ghx}{\hat{g}(x)}
\newcommand {\gh}{\hat{g}}
\newcommand {\gih}{\hat_i}
\newcommand {\gihx}{\hat{g_i}(x)}
%
\newcommand{\cmark}{\textcolor{green}{\ding{51}}}%
\newcommand{\xmark}{\textcolor{red}{\ding{55}}}%

\newcommand{\tr}{\operatorname{Tr}}
%

%
%
%

%
%
%
%
%

%
%

%

%
%
%
%
%


%

%
%
%


%

\newcommand*{\qedb}{\hfill\ensuremath{\square}}   %
\newcommand{\topic}[1]{\vspace{2mm}\noindent{{\bf #1:}}}
\newcommand{\head}[1]{\noindent{{\bf #1:}}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}

\newcommand{\zerosarah}{{\sf ZeroSARAH}\xspace}


==> KAUST_Thesis/imported/04_adaptive_clipping/import_setup.tex <==
%
%
\makeatletter
\let\as\@undefined
\let\asnote\@undefined
\let\AG\@undefined
\let\finf\@undefined
\let\prox\@undefined
\let\range\@undefined
\let\Comp\@undefined
\let\Comm\@undefined
\let\Span\@undefined
\let\Sp\@undefined
\let\Diag\@undefined
\let\diag\@undefined
\let\tr\@undefined
\let\cDb\@undefined
\let\Exp\@undefined
\let\ExpSub\@undefined
\let\ExpCond\@undefined
\let\bg\@undefined
\let\Rd\@undefined
\let\R\@undefined
\let\eps\@undefined
\let\tf\@undefined
\let\rnd\@undefined
\let\lmbdM\@undefined
\let\inner\@undefined
\let\shift\@undefined
\let\norm\@undefined
\let\normsq\@undefined
\let\vect\@undefined
\let\ecn\@undefined
\let\sqn\@undefined
\let\BB\@undefined
\let\CC\@undefined
\let\DD\@undefined
\let\EE\@undefined
\let\FF\@undefined
\let\GG\@undefined
\let\HH\@undefined
\let\II\@undefined
\let\JJ\@undefined
\let\KK\@undefined
\let\LL\@undefined
\let\MM\@undefined
\let\NN\@undefined
\let\OO\@undefined
\let\PP\@undefined
\let\QQ\@undefined
\let\RR\@undefined
\let\TT\@undefined
\let\UU\@undefined
\let\VV\@undefined
\let\WW\@undefined
\let\XX\@undefined
\let\YY\@undefined
\let\ZZ\@undefined
\let\cA\@undefined
\let\cB\@undefined
\let\cC\@undefined
\let\cD\@undefined
\let\cE\@undefined
\let\cF\@undefined
\let\cG\@undefined
\let\cH\@undefined
\let\cI\@undefined
\let\cJ\@undefined
\let\cK\@undefined
\let\cL\@undefined
\let\cM\@undefined
\let\cN\@undefined
\let\cO\@undefined
\let\cP\@undefined
\let\cQ\@undefined
\let\cR\@undefined
\let\cS\@undefined
\let\cT\@undefined
\let\cU\@undefined
\let\cV\@undefined
\let\cW\@undefined
\let\cX\@undefined
\let\cY\@undefined
\let\cZ\@undefined
\let\mA\@undefined
\let\mB\@undefined
\let\mC\@undefined
\let\mD\@undefined
\let\mE\@undefined
\let\mF\@undefined
\let\mG\@undefined
\let\mH\@undefined
\let\mI\@undefined
\let\mJ\@undefined
\let\mK\@undefined
\let\mL\@undefined
\let\mM\@undefined
\let\mN\@undefined
\let\mO\@undefined
\let\mP\@undefined
\let\mQ\@undefined
\let\mR\@undefined
\let\mS\@undefined
\let\mT\@undefined
\let\mU\@undefined
\let\mV\@undefined
\let\mW\@undefined
\let\mX\@undefined
\let\mY\@undefined
\let\mZ\@undefined
\let\mWp\@undefined
\let\sqnw\@undefined
\let\eqdef\@undefined
\let\br\@undefined
\let\sbr\@undefined
\let\cbr\@undefined
\let\bfL\@undefined
\let\bfC\@undefined
\let\mcL\@undefined
\let\mcB\@undefined
\let\cb\@undefined
\let\moL\@undefined
\let\moB\@undefined
\let\moD\@undefined
\let\moW\@undefined
\let\ob\@undefined
\let\oCb\@undefined
\let\bb\@undefined
\let\oDb\@undefined
\let\cbb\@undefined
\let\Var\@undefined
\let\argmin\@undefined
\makeatother
\input{KAUST_Thesis/imported/04_adaptive_clipping/source_macros}
\makeatletter
\let\oalpha\@undefined
\let\gf\@undefined
\let\Prob\@undefined
\let\algname\@undefined
\let\alg\@undefined
\let\sgd\@undefined
\let\circledOne\@undefined
\let\circledTwo\@undefined
\let\circledThree\@undefined
\makeatother
\newcommand{\oalpha}{\mathop{\overline{\alpha}}}
\newcommand{\gf}{\nabla f_\xi}
\newcommand{\Prob}{\mathrm{Prob}}
\definecolor{midnightblue}{HTML}{0059b3}
\newcommand{\algname}[1]{{\color{midnightblue!70!black}\small\sf#1}\xspace}
\newcommand{\alg}{\algname{QC-SGD}}
\newcommand{\sgd}{\algname{SGD}}
\newcommand{\circledOne}{\text{\large\ding{172}} }
\newcommand{\circledTwo}{\text{\large\ding{173}} }
\newcommand{\circledThree}{\text{\large \ding{174}} }
%
\mathchardef\epsilon="010F
\providecommand{\say}[1]{``#1''}
\makeatletter
\providecommand{\import@cite@plain}[1]{\cite{#1}}
\providecommand{\import@cite@opt}[1][]{\@ifnextchar[{\import@cite@opt@two}{\import@cite@opt@one}}
\providecommand{\import@cite@opt@one}[1]{\cite{#1}}
\providecommand{\import@cite@opt@two}[2][]{\cite{#2}}
\@ifundefined{citep}{\DeclareRobustCommand{\citep}{\@ifnextchar[{\import@cite@opt}{\import@cite@plain}}}{}
\@ifundefined{citet}{\DeclareRobustCommand{\citet}{\citep}}{}
\@ifundefined{citealp}{\DeclareRobustCommand{\citealp}{\citep}}{}
\@ifundefined{citealt}{\DeclareRobustCommand{\citealt}{\citep}}{}
\@ifundefined{citeauthor}{\DeclareRobustCommand{\citeauthor}{\citep}}{}
\@ifundefined{citeyear}{\DeclareRobustCommand{\citeyear}{\citep}}{}
\@ifundefined{citeyearpar}{\DeclareRobustCommand{\citeyearpar}{\citep}}{}
\makeatother
\providecommand{\Cref}[1]{\ref{#1}}
\providecommand{\cref}[1]{\ref{#1}}
\def\<#1,#2>{\langle #1,#2\rangle}


==> KAUST_Thesis/imported/04_adaptive_clipping/source_macros.tex <==
%
%
%
%
%
%
%


%
%
%
%
%
%
%
%

%
%
%

%
%
%
%

%

\newcommand{\as}[1]{{\color{green} #1}}
\newcommand{\asnote}[1]{\todo[color=green!]{#1}}

%

%
%
%
%
%
%
%

\newcommand{\AG}{\mathrm{AG}}

\newcommand{\finf}{f^{\mathrm{inf}}}

\newcommand{\prox}{\mathrm{prox}}
\newcommand{\range}{\mathrm{range}}
\newcommand{\Comp}{\mathrm{Comp}}
\newcommand{\Comm}{\mathrm{Comm}}
\newcommand{\Span}{\mathrm{Span}}
\newcommand{\Sp}{\mathrm{Sp}}

\newcommand{\Diag}{\mathrm{Diag}}
\newcommand{\diag}{\mathrm{diag}}

\newcommand{\tr}{\mathrm{tr}}

\newcommand{\bfL}{\mathop{\mathbf{L}}}
\newcommand{\bfC}{\mathop{\mathbf{C}}}
\newcommand{\mcL}{\mathop{\tilde{\mathbf{L}}}}
\newcommand{\mcB}{\mathop{\tilde{\mathbf{B}}}}
\newcommand{\cb}{\mathop{\tilde{\mathrm{b}}}}

\newcommand{\moL}{\mathop{\overline{\mathbf{L}}}}
\newcommand{\moB}{\mathop{\overline{\mathbf{B}}}}
\newcommand{\moD}{\mathop{\overline{\mathbf{D}}}}
\newcommand{\moW}{\mathop{\overline{\mathbf{W}}}}
\newcommand{\ob}{\mathop{\overline{b}}}
\newcommand{\oCb}{\mathop{\overline{\mathbf{C}b}}}

\newcommand{\bb}{\mathop{\mathrm{b}}}
\newcommand{\oDb}{\mathop{\overline{\mD^{-\frac{1}{2}}\bb}}}
\newcommand{\cDb}{\widetilde{\mD\bb}}
\newcommand{\cbb}{\mathop{\overline{\bb^{\frac{1}{2}}}}}



\newcommand{\Exp}[1]{{\color{black}  \mathbb{E}}\left[#1\right]}
\newcommand{\ExpSub}[2]{{\mathbb{E}}_{#1}\left[#2\right]}
\newcommand{\ExpCond}[2]{{\mathbb{E}}\left[\left.#1\right\vert#2\right]}
\newcommand{\Var}{\mathop{{\bf Var}}}

\newcommand{\bg}{\mathrm{D}}

\newcommand{\Rd}{\mathbb{R}^d}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\eps}{\varepsilon}

\def\<#1,#2>{\langle #1,#2\rangle}


\newcommand{\tf}{f_{\mathcal{D}}}
\newcommand{\rnd}[1]{{\texttt{Rand-}}#1}
\newcommand{\lmbdM}{\lambda_{\mathrm{m}}}


%

\newcommand{\inner}[2]{\left\langle #1 ,  #2 \right\rangle}

\definecolor{burgundy}{rgb}{0.5, 0.0, 0.13}
\definecolor{darkscarlet}{rgb}{0.34, 0.01, 0.1}
\newcommand{\shift}{{\color{purple}v}} 

%


\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\normsq}[1]{\norm{#1}^2}
\newcommand{\vect}[1]{\begin{bmatrix*}[l]#1\end{bmatrix*}}
\newcommand{\ecn}[1]{\Exp{\sqn{#1}}}

\newcommand\br[1]{\left( #1 \right)}
\newcommand\sbr[1]{\left[#1\right]}
\newcommand\cbr[1]{\left\{#1\right\}}

\newcommand{\sqn}[1]{\norm{#1}^2}



\newcommand{\BB}{\mathbb{B}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\DD}{\mathbb{D}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\FF}{\mathbb{F}}
\newcommand{\GG}{\mathbb{G}}
\newcommand{\HH}{\mathbb{H}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\JJ}{\mathbb{J}}
\newcommand{\KK}{\mathbb{K}}
\newcommand{\LL}{\mathbb{L}}
\newcommand{\MM}{\mathbb{M}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\OO}{\mathbb{O}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\TT}{\mathbb{T}}
\newcommand{\UU}{\mathbb{U}}
\newcommand{\VV}{\mathbb{V}}
\newcommand{\WW}{\mathbb{W}}
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\ZZ}{\mathbb{Z}}


\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\mA}{\mathbf{A}}
\newcommand{\mB}{\mathbf{B}}
\newcommand{\mC}{\mathbf{C}}
\newcommand{\mD}{\mathbf{D}}
\newcommand{\mE}{\mathbf{E}}
\newcommand{\mF}{\mathbf{F}}
\newcommand{\mG}{\mathbf{G}}
\newcommand{\mH}{\mathbf{H}}
\newcommand{\mI}{\mathbf{I}}
\newcommand{\mJ}{\mathbf{J}}
\newcommand{\mK}{\mathbf{K}}
\newcommand{\mL}{\mathbf{L}}
\newcommand{\mM}{\mathbf{M}}
\newcommand{\mN}{\mathbf{N}}
\newcommand{\mO}{\mathbf{O}}
\newcommand{\mP}{\mathbf{P}}
\newcommand{\mQ}{\mathbf{Q}}
\newcommand{\mR}{\mathbf{R}}
\newcommand{\mS}{\mathbf{S}}
\newcommand{\mT}{\mathbf{T}}
\newcommand{\mU}{\mathbf{U}}
\newcommand{\mV}{\mathbf{V}}
\newcommand{\mW}{\mathbf{W}}
\newcommand{\mX}{\mathbf{X}}
\newcommand{\mY}{\mathbf{Y}}
\newcommand{\mZ}{\mathbf{Z}}


\newcommand{\mWp}{\mathbf{W}^{\dagger}}


\newcommand{\sqnw}[1]{\sqn{#1}_{\mWp}}
\newcommand{\eqdef}{\coloneqq}
\newcommand{\argmin}{\operatorname*{arg\,min}}


==> KAUST_Thesis/imported/05_smoothed_normalization/import_setup.tex <==
%
%
\makeatletter
\let\Arg\@undefined
\let\B\@undefined
\let\Clip\@undefined
\let\Corr\@undefined
\let\Cov\@undefined
\let\Diag\@undefined
\let\E\@undefined
\let\Exp\@undefined
\let\ExpCond\@undefined
\let\ExpSub\@undefined
\let\Image\@undefined
\let\Ker\@undefined
\let\Normalize\@undefined
\let\PermComp\@undefined
\let\Prob\@undefined
\let\ProbCond\@undefined
\let\R\@undefined
\let\Sample\@undefined
\let\U\@undefined
\let\Var\@undefined
\let\abs\@undefined
\let\alg\@undefined
\let\algname\@undefined
\let\approxalg\@undefined
\let\bdry\@undefined
\let\cA\@undefined
\let\cB\@undefined
\let\cC\@undefined
\let\cD\@undefined
\let\cF\@undefined
\let\cH\@undefined
\let\cL\@undefined
\let\cN\@undefined
\let\cO\@undefined
\let\cQ\@undefined
\let\cS\@undefined
\let\cT\@undefined
\let\cW\@undefined
\let\cX\@undefined
\let\cY\@undefined
\let\cZ\@undefined
\let\card\@undefined
\let\cl\@undefined
\let\cmark\@undefined
\let\cone\@undefined
\let\conv\@undefined
\let\del\@undefined
\let\diag\@undefined
\let\diam\@undefined
\let\dom\@undefined
\let\done\@undefined
\let\egor\@undefined
\let\epi\@undefined
\let\eqdef\@undefined
\let\g\@undefined
\let\green\@undefined
\let\h\@undefined
\let\hotidea\@undefined
\let\inp\@undefined
\let\interior\@undefined
\let\la\@undefined
\let\lin\@undefined
\let\linspace\@undefined
\let\linspan\@undefined
\let\mD\@undefined
\let\mI\@undefined
\let\mJ\@undefined
\let\mL\@undefined
\let\mM\@undefined
\let\mN\@undefined
\let\mO\@undefined
\let\nnz\@undefined
\let\norm\@undefined
\let\nullspace\@undefined
\let\orange\@undefined
\let\peter\@undefined
\let\qedsymbol\@undefined
\let\ra\@undefined
\let\range\@undefined
\let\rank\@undefined
\let\red\@undefined
\let\ri\@undefined
\let\rint\@undefined
\let\sarit\@undefined
\let\signum\@undefined
\let\sqnorm\@undefined
\let\squeeze\@undefined
\let\st\@undefined
\let\theHalgorithm\@undefined
\let\todo\@undefined
\let\tr\@undefined
\let\vol\@undefined
\let\xmark\@undefined
\let\br\@undefined
\let\sbr\@undefined
\let\cbr\@undefined
\makeatother
\input{KAUST_Thesis/imported/05_smoothed_normalization/source_macros}
\makeatletter
\let\theHalgorithm\@undefined
\makeatother
\newcommand{\theHalgorithm}{\arabic{algorithm}}
%
%
\mathchardef\epsilon="010F
\makeatletter
\@ifundefined{lll}{}{\let\ll\lll}
\@ifundefined{ggg}{}{\let\gg\ggg}
\makeatother
\providecommand{\egor}[1]{}
\providecommand{\sarit}[1]{}
\providecommand{\peter}[1]{}
\providecommand{\todo}[2][]{}
\makeatletter
\providecommand{\import@cite@plain}[1]{\cite{#1}}
\providecommand{\import@cite@opt}[1][]{\@ifnextchar[{\import@cite@opt@two}{\import@cite@opt@one}}
\providecommand{\import@cite@opt@one}[1]{\cite{#1}}
\providecommand{\import@cite@opt@two}[2][]{\cite{#2}}
\@ifundefined{citep}{\DeclareRobustCommand{\citep}{\@ifnextchar[{\import@cite@opt}{\import@cite@plain}}}{}
\@ifundefined{citet}{\DeclareRobustCommand{\citet}{\citep}}{}
\@ifundefined{citealp}{\DeclareRobustCommand{\citealp}{\citep}}{}
\@ifundefined{citealt}{\DeclareRobustCommand{\citealt}{\citep}}{}
\@ifundefined{citeauthor}{\DeclareRobustCommand{\citeauthor}{\citep}}{}
\@ifundefined{citeyear}{\DeclareRobustCommand{\citeyear}{\citep}}{}
\@ifundefined{citeyearpar}{\DeclareRobustCommand{\citeyearpar}{\citep}}{}
\makeatother
\providecommand{\Cref}[1]{\ref{#1}}
\providecommand{\cref}[1]{\ref{#1}}
\providecommand{\say}[1]{``#1''}
\providecommand{\todo}[2][]{}
\providecommand{\qedsymbol}{$\square$}
\def\<#1,#2>{\langle #1,#2\rangle}


==> KAUST_Thesis/imported/05_smoothed_normalization/source_macros.tex <==
%

%
%

%
%
%
%
%

%
%
%
%
%
%

%
%
%
%
%
%
%

%
\newcommand{\g}{{\color{red}g}}
\newcommand{\h}{{\color{blue}h}}

%
\newcommand{\Clip}[2]{{\rm Clip}_{#1}\left( #2 \right)}
\newcommand{\Normalize}[2]{{\rm Norm}_{#1}\left( #2 \right)}


\newcommand{\abs}[1]{\left\vert #1 \right\vert}
\newcommand{\norm}[1]{\left\| #1 \right\|}
\newcommand{\sqnorm}[1]{\left\| #1 \right\|^2}
\newcommand{\lin}[1]{\left\langle #1\right\rangle} %
\newcommand{\inp}[2]{\left\langle#1,#2\right\rangle} %

\newcommand\br[1]{\left( #1 \right)} %
%
%
\newcommand\sbr[1]{\left[#1\right]}
\newcommand\cbr[1]{\left\{#1\right\}}

%
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

%
%
%
\newcommand{\mI}{\mathbf{I}}
%
%
%
%


%
\newcommand{\hotidea}{{\color{red}\bf HOT IDEA: }}
\newcommand{\done}{{\color{blue}\bf DONE: }}
\newcommand{\del}[1]{}
\let\la=\langle
\let\ra=\rangle

%
\definecolor{green}{rgb}{0.16, 0.67, 0.53}
\definecolor{lasallegreen}{rgb}{0.03, 0.47, 0.19}
\definecolor{midnightblue}{HTML}{0059b3}

%
%
%

\newcommand{\R}{\mathbb{R}} %
\newcommand{\U}{\mathbb{U}} %
\newcommand{\PermComp}{\U\mathbb{P}} %

\newcommand{\st}{\;:\;} %
%
\newcommand{\eqdef}{:=} %

\newcommand{\Prob}{\mathbf{Prob}} %
\newcommand{\ProbCond}[2]{\Prob\left(\left.#1\right\vert#2\right)}

\newcommand{\nnz}[1]{{\color{red}\|#1\|_0}}

%
\newcommand{\card}{\operatorname{card}}
\newcommand{\diam}{\operatorname{diam}}
\newcommand{\vol}{\operatorname{vol}}

%
\newcommand{\Exp}[1]{{\mathbb{E}}\left[#1\right]}
\newcommand{\ExpCond}[2]{{\mathbb{E}}\left[\left.#1\right\vert#2\right]}
\newcommand{\ExpSub}[2]{{\mathbb{E}}_{#1}\left[#2\right]}
\newcommand{\Cov}{\operatorname{Cov}}
\newcommand{\Var}{\operatorname{Var}}
\newcommand{\Corr}{\operatorname{Corr}}

%
\newcommand{\signum}{\operatorname{sign}}
\newcommand{\dom}{\operatorname{dom}}
\newcommand{\epi}{\operatorname{epi}}
\newcommand{\Ker}{\operatorname{null}}
\newcommand{\nullspace}{\operatorname{null}}
\newcommand{\range}{\operatorname{range}}
\newcommand{\Image}{\operatorname{Im}}

%
\newcommand{\interior}{\operatorname{int}}
\newcommand{\ri}{\operatorname{rint}}
\newcommand{\rint}{\operatorname{rint}}
\newcommand{\bdry}{\operatorname{bdry}}
\newcommand{\cl}{\operatorname{cl}}

%
\newcommand{\linspan}{\operatorname{span}}
\newcommand{\linspace}{\operatorname{linspace}}
\newcommand{\cone}{\operatorname{cone}}

\newcommand{\tr}{\operatorname{tr}}
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\conv}{\operatorname{conv}}
\newcommand{\Diag}{\operatorname{Diag}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\Arg}{\operatorname{Arg}}

%




%

%
\newcommand{\Sample}{\mathcal{S}}
%
%
\newcommand{\B}{\mathbb{B}}





%

%
%
%
%
%
%
%

%

%
%
%
%
%

%

%

%
%
%



%

%
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%

\definecolor{red}{rgb}{1.0, 0.01, 0.24}


\newcommand{\alg}{\textcolor{midnightblue!70!black}{\small\sf $\alpha$-NormEC}\xspace}

\newcommand{\algname}[1]{\textcolor{midnightblue!70!black}{\small\sf#1}}



%
%
%
%


%

%

\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%


%

%



==> KAUST_Thesis/imported/06_gluon/import_setup.tex <==
%
%
\makeatletter
\let\Arg\@undefined
\let\B\@undefined
\let\Corr\@undefined
\let\Cov\@undefined
\let\Diag\@undefined
\let\Exp\@undefined
\let\ExpCond\@undefined
\let\ExpSub\@undefined
\let\ExpSubCond\@undefined
\let\Expxi\@undefined
\let\I\@undefined
\let\Id\@undefined
\let\Image\@undefined
\let\Ker\@undefined
\let\N\@undefined
\let\PermComp\@undefined
\let\Prob\@undefined
\let\ProbCond\@undefined
\let\Proj\@undefined
\let\R\@undefined
\let\Sample\@undefined
\let\Teq\@undefined
\let\U\@undefined
\let\Var\@undefined
\let\Z\@undefined
\let\alg\@undefined
\let\alglinelabel\@undefined
\let\algname\@undefined
\let\algnameLarge\@undefined
\let\algnamefootnote\@undefined
\let\algnamelarge\@undefined
\let\algnamescript\@undefined
\let\algnamesmall\@undefined
\let\algnametiny\@undefined
\let\approxalg\@undefined
\let\argmax\@undefined
\let\argmin\@undefined
\let\bdry\@undefined
\let\binp\@undefined
\let\bnorm\@undefined
\let\bprox\@undefined
\let\brac\@undefined
\let\brox\@undefined
\let\cA\@undefined
\let\cB\@undefined
\let\cC\@undefined
\let\cD\@undefined
\let\cE\@undefined
\let\cF\@undefined
\let\cH\@undefined
\let\cJ\@undefined
\let\cK\@undefined
\let\cL\@undefined
\let\cN\@undefined
\let\cO\@undefined
\let\cQ\@undefined
\let\cS\@undefined
\let\cT\@undefined
\let\cU\@undefined
\let\cW\@undefined
\let\cX\@undefined
\let\cY\@undefined
\let\cZ\@undefined
\let\card\@undefined
\let\ceil\@undefined
\let\cl\@undefined
\let\clip\@undefined
\let\cmark\@undefined
\let\cone\@undefined
\let\conv\@undefined
\let\del\@undefined
\let\diag\@undefined
\let\diam\@undefined
\let\dom\@undefined
\let\done\@undefined
\let\drox\@undefined
\let\egor\@undefined
\let\epi\@undefined
\let\eqdef\@undefined
\let\fix\@undefined
\let\flr\@undefined
\let\g\@undefined
\let\grad\@undefined
\let\green\@undefined
\let\h\@undefined
\let\hf\@undefined
\let\hotidea\@undefined
\let\inp\@undefined
\let\interior\@undefined
\let\la\@undefined
\let\lin\@undefined
\let\linspace\@undefined
\let\linspan\@undefined
\let\lmo\@undefined
\let\mw\@undefined
\let\mx\@undefined
\let\nnz\@undefined
\let\norm\@undefined
\let\nullspace\@undefined
\let\orange\@undefined
\let\orth\@undefined
\let\parens\@undefined
\let\peter\@undefined
\let\prog\@undefined
\let\proj\@undefined
\let\prox\@undefined
\let\qedsymbol\@undefined
\let\ra\@undefined
\let\range\@undefined
\let\rank\@undefined
\let\red\@undefined
\let\ri\@undefined
\let\rint\@undefined
\let\sarit\@undefined
\let\sgrad\@undefined
\let\sign\@undefined
\let\sqnorm\@undefined
\let\squeeze\@undefined
\let\sri\@undefined
\let\st\@undefined
\let\supp\@undefined
\let\tablescriptsize\@undefined
\let\tablesmall\@undefined
\let\teqp\@undefined
\let\theHalgorithm\@undefined
\let\todo\@undefined
\let\tprox\@undefined
\let\tr\@undefined
\let\trbar\@undefined
\let\vol\@undefined
\let\xmark\@undefined
\let\zer\@undefined
\makeatother
\input{KAUST_Thesis/imported/06_gluon/source_macros}
\makeatletter
\let\theHalgorithm\@undefined
\makeatother
\newcommand{\theHalgorithm}{\arabic{algorithm}}

%
%
\mathchardef\epsilon="010F
\makeatletter
\@ifundefined{lll}{}{\let\ll\lll}
\@ifundefined{ggg}{}{\let\gg\ggg}
\makeatother

\makeatletter
\providecommand{\import@cite@plain}[1]{\cite{#1}}
\providecommand{\import@cite@opt}[1][]{\@ifnextchar[{\import@cite@opt@two}{\import@cite@opt@one}}
\providecommand{\import@cite@opt@one}[1]{\cite{#1}}
\providecommand{\import@cite@opt@two}[2][]{\cite{#2}}
\@ifundefined{citep}{\DeclareRobustCommand{\citep}{\@ifnextchar[{\import@cite@opt}{\import@cite@plain}}}{}
\@ifundefined{citet}{\DeclareRobustCommand{\citet}{\citep}}{}
\@ifundefined{citealp}{\DeclareRobustCommand{\citealp}{\citep}}{}
\@ifundefined{citealt}{\DeclareRobustCommand{\citealt}{\citep}}{}
\@ifundefined{citeauthor}{\DeclareRobustCommand{\citeauthor}{\citep}}{}
\@ifundefined{citeyear}{\DeclareRobustCommand{\citeyear}{\citep}}{}
\@ifundefined{citeyearpar}{\DeclareRobustCommand{\citeyearpar}{\citep}}{}
\makeatother
\providecommand{\Cref}[1]{\ref{#1}}
\providecommand{\cref}[1]{\ref{#1}}
\providecommand{\say}[1]{``#1''}
\providecommand{\todo}[2][]{}
\providecommand{\qedsymbol}{$\square$}
\def\<#1,#2>{\langle #1,#2\rangle}


==> KAUST_Thesis/imported/06_gluon/source_macros.tex <==
%

%
%

%
%
%
%
%

%
%
%
%
%
%
%
%

%
%
%
%
%
%

%
%
%
%
%

%

%

%
%
%

%
%
%
%
\newcommand{\h}{{\color{blue}h}}

%

\newcommand{\norm}[1]{\left\| #1 \right\|}
\newcommand{\bnorm}[1]{\left\| #1 \right\|_{\mB}}
\newcommand{\sqnorm}[1]{\left\| #1 \right\|^2}
\newcommand{\lin}[1]{\left\langle #1\right\rangle} %
\newcommand{\inp}[2]{\left\langle#1,#2\right\rangle} %
\newcommand{\binp}[2]{\left\langle#1,#2\right\rangle_{\mB}}

\newcommand{\parens}[1]{\left( #1 \right)}
\newcommand{\brac}[1]{\left\{ #1 \right\}}


%
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

%
\newcommand{\mx}{\mathbf{x}}
\newcommand{\mw}{\mathbf{w}}

\newcommand{\proj}{\textnormal{Proj}^{\perp}}
\newcommand{\trbar}{\overline{\textnormal{Tr}}}

\newcommand{\prox}{\textnormal{prox}}
\newcommand{\drox}{\textnormal{drox}}
\newcommand{\teqp}{t_\textnormal{prox}}
\newcommand{\Teq}{t^*}
\newcommand{\tprox}{t^{\prox}}

\newcommand{\squeeze}{\textstyle}

\newcommand{\flr}[1]{\left\lfloor #1\right\rfloor} 
%

\newcommand{\hf}{\hat{f}}


\newcommand{\supp}{\textnormal{supp}}
\newcommand{\prog}{\textnormal{prog}}

\newcommand{\grad}{\nabla}
\newcommand{\sgrad}{\widehat{\nabla}}
\newcommand{\bprox}{\textnormal{brox}_f^t}
\newcommand{\brox}[3]{\textnormal{brox}_{#1}^{#2}{(#3)}}

%
\newcommand{\hotidea}{{\color{red}\bf HOT IDEA: }}
\newcommand{\done}{{\color{blue}\bf DONE: }}
\newcommand{\del}[1]{}
\let\la=\langle
\let\ra=\rangle

%
\newcommand{\R}{\mathbb{R}} %
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\I}{\mathbb{I}}
\newcommand{\U}{\mathbb{U}}
\newcommand{\PermComp}{\U\mathbb{P}}

\newcommand{\st}{\;:\;} %
%
\newcommand{\eqdef}{:=} %


\newcommand{\clip}[1]{{\rm {\color{mydarkred}clip}_{\tau}}\left(#1\right)}


\newcommand{\nnz}[1]{{\color{red}\|#1\|_0}}

%
\newcommand{\card}{\operatorname{card}}
\newcommand{\diam}{\operatorname{diam}}
\newcommand{\vol}{\operatorname{vol}}

\newcommand{\orth}{\operatorname{orth}}

\newcommand{\Prob}[1]{{\mathbb{P}}\left(#1\right)} %
%
\newcommand{\ProbCond}[2]{\mathbf{Prob}\left(\left.#1\right\vert#2\right)}

\newcommand{\Id}[1]{{\mathbb{I}}\left(#1\right)} %

%
\newcommand{\Exp}[1]{{\mathbb{E}}\left[#1\right]}
\newcommand{\Expxi}[1]{{\mathbb{E}_{\xi}}\left[#1\right]}
\newcommand{\ExpCond}[2]{{\mathbb{E}}\left[\left.#1\right\vert#2\right]}
\newcommand{\ExpSub}[2]{{\mathbb{E}}_{#1}\left[#2\right]}
\newcommand{\ExpSubCond}[3]{{\mathbb{E}}_{#1}\left[#2\vert#3\right]}
%
%
\newcommand{\Corr}{\operatorname{Corr}}

%
%
\newcommand{\dom}{\operatorname{dom}}
\newcommand{\epi}{\operatorname{epi}}
\newcommand{\Ker}{\operatorname{null}}
\newcommand{\nullspace}{\operatorname{null}}
\newcommand{\range}{\operatorname{range}}
\newcommand{\Image}{\operatorname{Im}}

%
\newcommand{\interior}{\operatorname{int}}
%
\newcommand{\sri}{\operatorname{sri}}
\newcommand{\rint}{\operatorname{rint}}
\newcommand{\bdry}{\operatorname{bdry}}
\newcommand{\cl}{\operatorname{cl}}
\newcommand{\zer}{\operatorname{zer}}
%

%
\newcommand{\linspan}{\operatorname{span}}
\newcommand{\linspace}{\operatorname{linspace}}
\newcommand{\cone}{\operatorname{cone}}

\newcommand{\tr}{\operatorname{tr}}
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\conv}{\operatorname{conv}}
\newcommand{\Diag}{\operatorname{Diag}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\Arg}{\operatorname{Arg}}
%
%

%




%

%
\newcommand{\Sample}{\mathcal{S}}
%
\newcommand{\B}{\mathbb{B}}


%
%
\definecolor{mydarkgreen}{RGB}{39,130,67}
\definecolor{mydarkred}{RGB}{192,47,25}
\definecolor{mydarkorange}{RGB}{39,130,67}
\newcommand{\green}{\color{mydarkgreen}}
\newcommand{\red}{\color{mydarkred}}
\newcommand{\cmark}{\green\ding{51}}%
\newcommand{\xmark}{\red\ding{55}}%
\newcommand{\orange}{\color{mydarkorange}}

\newcommand{\algnametiny}[1]{{\tiny \sf #1}}
\newcommand{\algnamescript}[1]{{\scriptsize \sf #1}}
\newcommand{\algnamefootnote}[1]{{\footnotesize \sf #1}}
\newcommand{\algname}[1]{{\small \sf #1}}
%
%
%

\newcommand{\tablescriptsize}[1]{{\scriptsize #1}}
\newcommand{\tablesmall}[1]{{\small #1}}



%

%
%
%
%
%
%
%
%

%
%
%
%
%
%

%
%
%
%
%
%

%
\newcommand{\alglinelabel}{%
  \addtocounter{ALC@line}{-1}%
  \refstepcounter{ALC@line}%
  \label%
}

%
%
%

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}
\definecolor{darkscarlet}{rgb}{0.34, 0.01, 0.1}
\definecolor{yaleblue}{rgb}{0.06, 0.3, 0.57}
\definecolor{darkpowderblue}{rgb}{0.0, 0.2, 0.6}
\definecolor{midnightblue}{HTML}{0059b3}
\definecolor{noonblue}{HTML}{e5eef7}
\definecolor{chromered}{HTML}{f14233}
\definecolor{olivedrab}{HTML}{6b8e23}
\definecolor{bgcolor}{rgb}{0.8,1,1}

\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\ttfamily\footnotesize,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2
}

\lstset{style=mystyle}

\newcommand{\lmo}[2]{{\rm LMO}_{#1}(#2)}
\newcommand{\Proj}[2]{\Pi_{#1}(#2)}

\newcommand{\argmax}{\operatorname*{arg\,max}}
\newcommand{\argmin}{\operatorname*{arg\,min}}


==> KAUST_Thesis/imported/07_beyond_the_ideal/import_setup.tex <==
%
%
\makeatletter
\let\Arg\@undefined
\let\B\@undefined
\let\BMoreau\@undefined
\let\BMoreauSub\@undefined
\let\BProx\@undefined
\let\BProxSub\@undefined
\let\Bpprox\@undefined
\let\BpproxSub\@undefined
\let\CBProxSub\@undefined
\let\Corr\@undefined
\let\Cov\@undefined
\let\Diag\@undefined
\let\Dprox\@undefined
\let\DproxSub\@undefined
\let\Exp\@undefined
\let\ExpCond\@undefined
\let\ExpSub\@undefined
\let\ExpSubCond\@undefined
\let\Expxi\@undefined
\let\I\@undefined
\let\Id\@undefined
\let\Image\@undefined
\let\Ker\@undefined
\let\MoreauSub\@undefined
\let\N\@undefined
\let\NBProxSub\@undefined
\let\PermComp\@undefined
\let\Prob\@undefined
\let\ProbCond\@undefined
\let\Proj\@undefined
\let\ProxSub\@undefined
\let\R\@undefined
\let\SBProjProxSub\@undefined
\let\SBProxSub\@undefined
\let\Sample\@undefined
\let\Sprox\@undefined
\let\SproxSub\@undefined
\let\Teq\@undefined
\let\U\@undefined
\let\Var\@undefined
\let\Z\@undefined
\let\alg\@undefined
\let\alglinelabel\@undefined
\let\algname\@undefined
\let\algnameLarge\@undefined
\let\algnamefootnote\@undefined
\let\algnamelarge\@undefined
\let\algnamescript\@undefined
\let\algnamesmall\@undefined
\let\algnametiny\@undefined
\let\approxalg\@undefined
\let\argmax\@undefined
\let\argmin\@undefined
\let\bdry\@undefined
\let\binp\@undefined
\let\bnorm\@undefined
\let\bprox\@undefined
\let\brac\@undefined
\let\breg\@undefined
\let\brox\@undefined
\let\cA\@undefined
\let\cB\@undefined
\let\cC\@undefined
\let\cD\@undefined
\let\cE\@undefined
\let\cF\@undefined
\let\cH\@undefined
\let\cJ\@undefined
\let\cK\@undefined
\let\cL\@undefined
\let\cN\@undefined
\let\cO\@undefined
\let\cQ\@undefined
\let\cS\@undefined
\let\cT\@undefined
\let\cU\@undefined
\let\cW\@undefined
\let\cX\@undefined
\let\cY\@undefined
\let\cZ\@undefined
\let\card\@undefined
\let\cbrac\@undefined
\let\ceil\@undefined
\let\cl\@undefined
\let\clip\@undefined
\let\cmark\@undefined
\let\cmax\@undefined
\let\cmin\@undefined
\let\cone\@undefined
\let\conv\@undefined
\let\del\@undefined
\let\diag\@undefined
\let\diam\@undefined
\let\dist\@undefined
\let\dom\@undefined
\let\done\@undefined
\let\drox\@undefined
\let\egor\@undefined
\let\epi\@undefined
\let\eqdef\@undefined
\let\fix\@undefined
\let\flr\@undefined
\let\g\@undefined
\let\grad\@undefined
\let\green\@undefined
\let\h\@undefined
\let\hf\@undefined
\let\hotidea\@undefined
\let\inner\@undefined
\let\inp\@undefined
\let\interior\@undefined
\let\la\@undefined
\let\lin\@undefined
\let\linspace\@undefined
\let\linspan\@undefined
\let\lmo\@undefined
\let\mA\@undefined
\let\mB\@undefined
\let\mC\@undefined
\let\mD\@undefined
\let\mH\@undefined
\let\mI\@undefined
\let\mJ\@undefined
\let\mL\@undefined
\let\mM\@undefined
\let\mN\@undefined
\let\mO\@undefined
\let\mP\@undefined
\let\mQ\@undefined
\let\mS\@undefined
\let\mT\@undefined
\let\mU\@undefined
\let\mV\@undefined
\let\mW\@undefined
\let\mX\@undefined
\let\mZ\@undefined
\let\mw\@undefined
\let\mx\@undefined
\let\nnz\@undefined
\let\norm\@undefined
\let\nullspace\@undefined
\let\orange\@undefined
\let\orth\@undefined
\let\parens\@undefined
\let\peter\@undefined
\let\prog\@undefined
\let\proj\@undefined
\let\prox\@undefined
\let\qedsymbol\@undefined
\let\ra\@undefined
\let\range\@undefined
\let\rank\@undefined
\let\rbrac\@undefined
\let\red\@undefined
\let\ri\@undefined
\let\rint\@undefined
\let\sarit\@undefined
\let\sbrac\@undefined
\let\sgrad\@undefined
\let\sign\@undefined
\let\sqnorm\@undefined
\let\squeeze\@undefined
\let\sri\@undefined
\let\st\@undefined
\let\supp\@undefined
\let\tablescriptsize\@undefined
\let\tablesmall\@undefined
\let\teqp\@undefined
\let\theHalgorithm\@undefined
\let\todo\@undefined
\let\tprox\@undefined
\let\tr\@undefined
\let\trbar\@undefined
\let\vol\@undefined
\let\xmark\@undefined
\let\zer\@undefined
\makeatother
\input{KAUST_Thesis/imported/07_beyond_the_ideal/source_macros}
\makeatletter
\let\algname\@undefined
\let\err\@undefined
\let\squeeze\@undefined
\let\approxalg\@undefined
\makeatother
\newcommand{\err}{\delta}
\newcommand{\squeeze}{\textstyle}
\definecolor{midnightblue}{rgb}{0.1,0.1,0.44}
\newcommand{\algname}[1]{{\color{midnightblue!70!black}\sf #1}}
\newcommand{\approxalg}[1]{{\ttfamily\color{midnightblue!70!black}#1}}
\makeatletter
\@ifundefined{algorithmicrequire}{\newcommand{\algorithmicrequire}{\textbf{Input:}}}{}
\makeatother
\makeatletter
\providecommand{\import@cite@plain}[1]{\cite{#1}}
\providecommand{\import@cite@opt}[1][]{\@ifnextchar[{\import@cite@opt@two}{\import@cite@opt@one}}
\providecommand{\import@cite@opt@one}[1]{\cite{#1}}
\providecommand{\import@cite@opt@two}[2][]{\cite{#2}}
\@ifundefined{citep}{\DeclareRobustCommand{\citep}{\@ifnextchar[{\import@cite@opt}{\import@cite@plain}}}{}
\@ifundefined{citet}{\DeclareRobustCommand{\citet}{\citep}}{}
\@ifundefined{citealp}{\DeclareRobustCommand{\citealp}{\citep}}{}
\@ifundefined{citealt}{\DeclareRobustCommand{\citealt}{\citep}}{}
\@ifundefined{citeauthor}{\DeclareRobustCommand{\citeauthor}{\citep}}{}
\@ifundefined{citeyear}{\DeclareRobustCommand{\citeyear}{\citep}}{}
\@ifundefined{citeyearpar}{\DeclareRobustCommand{\citeyearpar}{\citep}}{}
\makeatother
\providecommand{\Cref}[1]{\ref{#1}}
\providecommand{\cref}[1]{\ref{#1}}
\providecommand{\say}[1]{``#1''}
\providecommand{\todo}[2][]{}
\providecommand{\qedsymbol}{$\square$}
\def\<#1,#2>{\langle #1,#2\rangle}


==> KAUST_Thesis/imported/07_beyond_the_ideal/source_macros.tex <==
%

%
%

%
%
%
%
%

%
%
%
%
%
%
%
%

%

%

%
%
%
%
%

%

%

%
%
%

%
%
%
\newcommand{\h}{{\color{blue}h}}

%

\newcommand{\norm}[1]{\left\| #1 \right\|}
\newcommand{\bnorm}[1]{\left\| #1 \right\|_{\mB}}
\newcommand{\sqnorm}[1]{\left\| #1 \right\|^2}
\newcommand{\lin}[1]{\left\langle #1\right\rangle} %
\newcommand{\inp}[2]{\left\langle#1,#2\right\rangle} %
\newcommand{\binp}[2]{\left\langle#1,#2\right\rangle_{\mB}}

\newcommand{\parens}[1]{\left( #1 \right)}
\newcommand{\brac}[1]{\left\{ #1 \right\}}


%
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

%
\newcommand{\mA}{\mathbf{A}}
\newcommand{\mB}{\mathbf{B}}
\newcommand{\mC}{\mathbf{C}}
\newcommand{\mM}{\mathbf{M}}
\newcommand{\mN}{\mathbf{N}}
\newcommand{\mI}{\mathbf{I}}
\newcommand{\mJ}{\mathbf{J}}
\newcommand{\mL}{\mathbf{L}}
\newcommand{\mD}{\mathbf{D}}
\newcommand{\mO}{\mathbf{O}}
\newcommand{\mH}{\mathbf{H}}
\newcommand{\mP}{\mathbf{P}}
\newcommand{\mS}{\mathbf{S}}
\newcommand{\mT}{\mathbf{T}}
\newcommand{\mZ}{\mathbf{Z}}
\newcommand{\mU}{\mathbf{U}}
\newcommand{\mQ}{\mathbf{Q}}
\newcommand{\mV}{\mathbf{V}}
\newcommand{\mX}{\mathbf{X}}
\newcommand{\mW}{\mathbf{W}}

%
\newcommand{\mx}{\mathbf{x}}
\newcommand{\mw}{\mathbf{w}}

\newcommand{\proj}{\textnormal{Proj}^{\perp}}
\newcommand{\trbar}{\overline{\textnormal{Tr}}}

\newcommand{\prox}{\textnormal{prox}}
\newcommand{\drox}{\textnormal{drox}}
\newcommand{\teqp}{t_\textnormal{prox}}
\newcommand{\Teq}{t^*}
\newcommand{\tprox}{t^{\prox}}

%

\newcommand{\flr}[1]{\left\lfloor #1\right\rfloor} 
\newcommand{\ceil}[1]{\left\lceil #1\right\rceil} 

\newcommand{\hf}{\hat{f}}


\newcommand{\supp}{\textnormal{supp}}
\newcommand{\prog}{\textnormal{prog}}

\newcommand{\grad}{\nabla}
\newcommand{\sgrad}{\widehat{\nabla}}
\newcommand{\bprox}{\textnormal{brox}_f^t}
\newcommand{\brox}[3]{\textnormal{brox}_{#1}^{#2}{(#3)}}

%
\newcommand{\hotidea}{{\color{red}\bf HOT IDEA: }}
\newcommand{\done}{{\color{blue}\bf DONE: }}
\newcommand{\del}[1]{}
\let\la=\langle
\let\ra=\rangle

%
\newcommand{\R}{\mathbb{R}} %
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\I}{\mathbb{I}}
\newcommand{\U}{\mathbb{U}}
\newcommand{\PermComp}{\U\mathbb{P}}

\newcommand{\st}{\;:\;} %
%
\newcommand{\eqdef}{:=} %


\newcommand{\clip}[1]{{\rm {\color{mydarkred}clip}_{\tau}}\left(#1\right)}


\newcommand{\nnz}[1]{{\color{red}\|#1\|_0}}

%
\newcommand{\card}{\operatorname{card}}
\newcommand{\diam}{\operatorname{diam}}
\newcommand{\vol}{\operatorname{vol}}

\newcommand{\orth}{\operatorname{orth}}

\newcommand{\Prob}[1]{{\mathbb{P}}\left(#1\right)} %
%
\newcommand{\ProbCond}[2]{\mathbf{Prob}\left(\left.#1\right\vert#2\right)}

\newcommand{\Id}[1]{{\mathbb{I}}\left(#1\right)} %

%
\newcommand{\Exp}[1]{{\mathbb{E}}\left[#1\right]}
\newcommand{\Expxi}[1]{{\mathbb{E}_{\xi}}\left[#1\right]}
\newcommand{\ExpCond}[2]{{\mathbb{E}}\left[\left.#1\right\vert#2\right]}
\newcommand{\ExpSub}[2]{{\mathbb{E}}_{#1}\left[#2\right]}
\newcommand{\ExpSubCond}[3]{{\mathbb{E}}_{#1}\left[#2\vert#3\right]}
\newcommand{\Cov}{\operatorname{Cov}}
\newcommand{\Var}{\operatorname{Var}}
\newcommand{\Corr}{\operatorname{Corr}}

%
\newcommand{\sign}{\operatorname{sign}}
\newcommand{\dom}{\operatorname{dom}}
\newcommand{\epi}{\operatorname{epi}}
\newcommand{\Ker}{\operatorname{null}}
\newcommand{\nullspace}{\operatorname{null}}
\newcommand{\range}{\operatorname{range}}
\newcommand{\Image}{\operatorname{Im}}

%
\newcommand{\interior}{\operatorname{int}}
\newcommand{\ri}{\operatorname{ri}}
\newcommand{\sri}{\operatorname{sri}}
\newcommand{\rint}{\operatorname{rint}}
\newcommand{\bdry}{\operatorname{bdry}}
\newcommand{\cl}{\operatorname{cl}}
\newcommand{\zer}{\operatorname{zer}}
\newcommand{\fix}{\operatorname{Fix}}

%
\newcommand{\linspan}{\operatorname{span}}
\newcommand{\linspace}{\operatorname{linspace}}
\newcommand{\cone}{\operatorname{cone}}

\newcommand{\tr}{\operatorname{tr}}
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\conv}{\operatorname{conv}}
\newcommand{\Diag}{\operatorname{Diag}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\Arg}{\operatorname{Arg}}
\newcommand{\argmin}{\operatorname*{arg\,min}}
\newcommand{\argmax}{\operatorname*{arg\,max}}

%




%

%
\newcommand{\Sample}{\mathcal{S}}
%
\newcommand{\B}{\mathbb{B}}


%
%
\definecolor{mydarkgreen}{RGB}{39,130,67}
\definecolor{mydarkred}{RGB}{192,47,25}
\definecolor{mydarkorange}{RGB}{39,130,67}
\newcommand{\green}{\color{mydarkgreen}}
\newcommand{\red}{\color{mydarkred}}
\newcommand{\cmark}{\green\ding{51}}%
\newcommand{\xmark}{\red\ding{55}}%
\newcommand{\orange}{\color{mydarkorange}}

%
\newcommand{\algnametiny}[1]{{\tiny \red\sf #1}}
\newcommand{\algnamescript}[1]{{\scriptsize \red\sf #1}}
\newcommand{\algnamefootnote}[1]{{\footnotesize \red\sf #1}}
\newcommand{\algname}[1]{{\small \red \sf #1}}
%
%
%

\newcommand{\tablescriptsize}[1]{{\scriptsize #1}}
\newcommand{\tablesmall}[1]{{\small #1}}



%

%
%
%
%
%
%
%
%

%
%
%
%
%
%

%
%
%
%
%
%

%
\newcommand{\alglinelabel}{%
  \addtocounter{ALC@line}{-1}%
  \refstepcounter{ALC@line}%
  \label%
}

%
%
%

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}

\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\ttfamily\footnotesize,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2
}

\lstset{style=mystyle}

%
\newcommand{\rbrac}[1]{\left(#1\right)}
\newcommand{\sbrac}[1]{\left[#1\right]}
\newcommand{\cbrac}[1]{\left\{#1\right\}}
\newcommand{\BProx}{\textnormal{brox}}
\newcommand{\BProxSub}[3]{\textnormal{{brox}}^{#1}_{#2}(#3)}
\newcommand{\ProxSub}[2]{\textnormal{{prox}}_{#1}(#2)}
\newcommand{\MoreauSub}[3]{{M}^{#1}_{#2}\rbrac{#3}}
\newcommand{\BMoreauSub}[3]{{N}^{#1}_{#2}\rbrac{#3}}
\newcommand{\BMoreau}{{N}}
\newcommand{\inner}[2]{\left\langle #1, #2 \right\rangle}
\newcommand{\dist}[2]{\textnormal{dist}\rbrac{#1, #2}}
\newcommand{\breg}[3]{D_{#1}\rbrac{#2, #3}}
\newcommand{\cmin}[1]{c^{\min}_t\rbrac{x_{#1}}}
\newcommand{\cmax}[1]{c^{\max}_t\rbrac{x_{#1}}}
\newcommand{\BpproxSub}[3]{\textnormal{{bprox}}^{#1}_{#2}\left(#3\right)}
\newcommand{\Bpprox}{\textnormal{bprox}}
\newcommand{\Sprox}{\textnormal{{Sprox}}}
\newcommand{\SproxSub}[4]{\textnormal{{Sprox}}^{#1}_{#2, #3}\rbrac{#4}}
\newcommand{\Dprox}{\textnormal{dprox}}
\newcommand{\DproxSub}[3]{\textnormal{dprox}^{#1}_{#2, #3}}
\newcommand{\SBProjProxSub}[3]{\Pi\rbrac{#3, \BProxSub{#1}{#2}{#3}}}

\newcommand{\CBProxSub}[3]{\textnormal{{cbrox}}^{#1}_{#2}(#3)}
\newcommand{\NBProxSub}[3]{\textnormal{{nbrox}}^{#1}_{#2}(#3)}
\newcommand{\SBProxSub}[3]{\textnormal{{sbrox}}^{#1}_{#2}(#3)}
\newcommand{\lmo}[2]{{\rm LMO}_{#1}(#2)}
\newcommand{\Proj}[2]{\Pi_{#1}(#2)}
